Bootstrapping $N_f=4$ conformal QED$_3$

We present the results of a conformal bootstrap study of the presumed unitary IR fixed point of quantum electrodynamics in three dimensions (QED$_3$) coupled to $N_f=4$ two-component Dirac fermions. Specifically, we study the four-point correlators of the $SU(4)$ adjoint fermion bilinear $r$ and the monopole of lowest topological charge $\mathcal{M}_{1/2}$. Most notably, the scaling dimensions of the fermion bilinear $r$ and the monopole $\mathcal{M}_{1/2}$ are found to be constrained into a closed island with a combination of spectrum assumptions inspired by the $1/N_f$ perturbative results as well as a novel interval positivity constraint on the next-lowest-charge monopole $\mathcal{M}_1$. Bounds in this island on the $SU(4)$ and topological $U(1)_t$ conserved current central charges $c_J$, $c_J^t$, as well as on the stress tensor central charge $c_T$, are comfortably consistent with the perturbative results. Together with the scaling dimensions, this suggests that a part of estimates from the $1/N_f$ expansion -- even at $N_f=4$ -- provide a self-consistent solution to the bootstrap crossing relations, despite some of our assumptions not being strictly justified.

==> Revtex Version/table_mixed.tex <==
\begin{table}
	\centering
\caption{\label{tab:summarize-SU4}
	A summary of the conformal blocks and the OPE coefficients in the SU(4) mixed monopole-fermion-bilinear correlators.}

\begin{tabular}{ccccc}
\hline\hline\\[-1em]
$\SU(4)$ \textbf{name}& \textbf{Young tableaux} & $\SO(2)$ \textbf{rep} & \textbf{Spin} & \textbf{OPE}
\\[.1em]\hline\\[-1em]
		$\begin{array}{c}\mathsf{Singlet}\\{(000)}\end{array} $ 
	& $\bullet$ 
	& $\begin{array}{c}S\\A\\T\end{array}$
	&\begin{tabular}{l}even\\odd\\even\end{tabular} 
	&$\begin{array}{l}
		\lambda _{rrO},\lambda _{MMO} \\
		\lambda _{MMO} \\
		\lambda _{MMO} \\
		\end{array}$
\\[.1em]\hline\\[-1em]	
		$\begin{array}{c}\mathsf{Adj}\\{(211)}\end{array} $
	&$\raisebox{-1.2em}{\includegraphics[width=1.6em]{young-tabs/Adj-small}}$
	&$\begin{array}{c}
		S \\
		S \\
		A \\
		T \\
		\end{array}$
	&\begin{tabular}{l}odd\\even\\even\\odd\end{tabular}
	& $\begin{array}{l}
		\lambda _{rrO},\lambda _{MMO} \\
		\lambda _{rrO} \\
		\lambda _{MMO} \\
		\lambda _{MMO} \\
	\end{array}$
\\[.1em]\hline\\[-1em]	
		$\begin{array}{c}\mathsf{AA}\\{(220)}\end{array} $		
	&$\raisebox{-.8em}{\includegraphics[width=1.6em]{young-tabs/AA-small}}$
	&$	\begin{array}{c}
		S \\
		A \\
		T \\
	\end{array}$
	&\begin{tabular}{l}even\\odd\\even	\end{tabular}
	&$	\begin{array}{l}
		\lambda _{rrO},\lambda _{MMO} \\
		\lambda _{MMO} \\
		\lambda _{MMO} \\
		\end{array}$
\\[.1em]\hline\\[-1em]	
		$\begin{array}{c}\mathsf{S \bar{A} }\\{(310)_R}\end{array}$
	&$\raisebox{-1.2em}{\includegraphics[width=2.4em]{young-tabs/ASb-small}}$
	&$S$
	&\begin{tabular}{l}odd\end{tabular}
	&$\begin{array}{l}
		\lambda _{rrO}\color{white}{,\lambda _{MMO}}
		\end{array}$
\\[.1em]\hline\\[-1em]	
		$\begin{array}{c}\mathsf{ S \bar{S} }\\{(422)}\end{array} $
	&$\raisebox{-1.2em}{\includegraphics[width=3.2em]{young-tabs/SSb-small}}$
	&$S$
	&\begin{tabular}{l}even	\end{tabular}
	&$\begin{array}{l}
		\lambda _{rrO}\color{white}{,\lambda _{MMO}}
		\end{array}$
\\[.1em]\hline\\[-1em]	
	$\begin{array}{c}\mathsf{Anti}\\{(110)}\end{array} $
	&$\raisebox{-.8em}{\includegraphics[width=.8em]{young-tabs/A-small}}$
	&$V$
	&\begin{tabular}{l}both	\end{tabular}
	& $\begin{array}{l}
		\lambda _{rMO}\color{white}{,\lambda _{MMO}}
	\end{array}$
\\[.1em]\hline\\[-1em]	
	$\begin{array}{c}\mathsf{Sym}\\{(200)}\end{array}$
	&$\raisebox{-.4em}{\includegraphics[width=1.6em]{young-tabs/S-small}}$
	&$V$
	&\begin{tabular}{l}both	\end{tabular}
	& $\begin{array}{l}
		\lambda _{rMO}\color{white}{,\lambda _{MMO}}
	\end{array}$
\\[.1em]\hline\\[-1em]	
	$\begin{array}{c}\mathsf{AAdj}\\{(321)}\end{array} $
	&$	\raisebox{-1.2em}{\includegraphics[width=2.4em]{young-tabs/AAdj-small}}$
	&$V$
	&\begin{tabular}{l}both	\end{tabular}
	& $\begin{array}{l}
		\lambda _{rMO}\color{white}{,\lambda _{MMO}}
	\end{array}$
\\[.1em]\hline\hline
\end{tabular}
\end{table}
\iffalse 
\begin{table}[ht!]
	\centering
	$$
	\begin{array}{|l|c|c|c|l|}
		\hline
		\text{SU(4)} &
		\text{name} & \text{SO(2)} & \text{spin} & ~~~~~\text{OPE}   \\
		\hline
		\cdot &
		\begin{array}{c}\mathsf{0}\\{(000)}\end{array} & 
		\begin{array}{c}
			S \\
			A \\
			T \\
		\end{array}
		& 
		\begin{array}{c}
			\text{even} \\
			\text{odd} \\
			\text{even} \\
		\end{array}
		& 
		\begin{array}{l}
			\lambda _{rrO},\lambda _{MMO} \\
			\lambda _{MMO} \\
			\lambda _{MMO} \\
		\end{array}
		\\
		\hline
		\raisebox{-1.2em}{\includegraphics[width=1.6em]{young-tabs/Adj-small}}&
		\begin{array}{c}\mathsf{Adj}\\{(211)}\end{array} & 
		\begin{array}{c}
			S \\
			S \\
			A \\
			T \\
		\end{array}
		& 
		\begin{array}{l}
			\text{odd} \\
			\text{even} \\
			\text{even} \\
			\text{odd} \\
		\end{array}
		& 
		\begin{array}{l}
			\lambda _{rrO},\lambda _{MMO} \\
			\lambda _{rrO} \\
			\lambda _{MMO} \\
			\lambda _{MMO} \\
		\end{array}
		\\
		\hline
		\raisebox{-.8em}{\includegraphics[width=1.6em]{young-tabs/AA-small}}&
		\begin{array}{c}\mathsf{AA}\\{(220)}\end{array} & 
		\begin{array}{c}
			S \\
			A \\
			T \\
		\end{array}
		& 
		\begin{array}{c}
			\text{even} \\
			\text{odd} \\
			\text{even} \\
		\end{array}
		& 
		\begin{array}{l}
			\lambda _{rrO},\lambda _{MMO} \\
			\lambda _{MMO} \\
			\lambda _{MMO} \\
		\end{array}
		\\
		\hline
		\raisebox{-1.2em}{\includegraphics[width=2.4em]{young-tabs/ASb-small}}&
		\begin{array}{c}\mathsf{A \bar{S} }\\{(220)}\end{array} & 
		\begin{array}{c}
			S \\
		\end{array}
		& 
		\begin{array}{c}
			\text{odd} \\
		\end{array}
		& 
		\begin{array}{l}
			\lambda _{rrO} \\
		\end{array}
		\\
		%  \hline
		%  \raisebox{-.8em}{\includegraphics[width=2.4em]{figs/AS-small}}&
		%  \mathsf{\left(A \bar{S}\right)^{\dagger } }& 
		% \begin{array}{c}
		%  S \\
		% \end{array}
		%  & 
		% \begin{array}{c}
		%  \text{odd} \\
		% \end{array}
		%  & 
		% \begin{array}{l}
		%  \lambda _{rrO} \\
		% \end{array}
		%  \\
		\hline
		\raisebox{-1.2em}{\includegraphics[width=3.2em]{young-tabs/SSb-small}}&
		\begin{array}{c}\mathsf{ S \bar{S} }\\{(422)}\end{array} & 
		\begin{array}{c}
			S \\
		\end{array}
		& 
		\begin{array}{c}
			\text{even} \\
		\end{array}
		& 
		\begin{array}{l}
			\lambda _{rrO} \\
		\end{array}
		\\
		\hline
		\raisebox{-.8em}{\includegraphics[width=.8em]{young-tabs/A-small}}&
		\begin{array}{c}\mathsf{Anti}\\{(110)}\end{array} & 
		\begin{array}{c}
			V \\
		\end{array}
		& 
		\begin{array}{c}
			\text{both} \\
		\end{array}
		& 
		\begin{array}{l}
			\lambda _{rMO} \\
		\end{array}
		\\
		%  \hline
		%  \raisebox{-1.2em}{\includegraphics[width=1.6em]{figs/Sb-small}}&
		%  \mathsf{\bar{S}} & 
		% \begin{array}{c}
		%  V \\
		% \end{array}
		%  & 
		% \begin{array}{c}
		%  \text{both} \\
		% \end{array}
		%  & 
		% \begin{array}{l}
		%  \lambda _{rMO} \\
		% \end{array}
		%  \\
		\hline
		\raisebox{-.4em}{\includegraphics[width=1.6em]{young-tabs/S-small}}&
		\begin{array}{c}\mathsf{Sym}\\{(200)}\end{array} & 
		\begin{array}{c}
			V \\
		\end{array}
		& 
		\begin{array}{c}
			\text{both} \\
		\end{array}
		& 
		\begin{array}{l}
			\lambda _{rMO} \\
		\end{array}
		\\
		\hline
		\raisebox{-1.2em}{\includegraphics[width=2.4em]{young-tabs/AAdj-small}}&
		\begin{array}{c}\mathsf{AAdj}\\{(321)}\end{array} & 
		\begin{array}{c}
			V \\
		\end{array}
		& 
		\begin{array}{c}
			\text{both} \\
		\end{array}
		& 
		\begin{array}{l}
			\lambda _{rMO} \\
		\end{array}
		\\
		\hline
	\end{array}
	$$
	\caption{\label{tab:summarize-SU4}
		A summary of the conformal blocks and the OPE coefficients in the SU(4) mixed monopole-fermion-bilinear correlators.}
\end{table}
\fi 
